Supporting Changes in Digital Ownership and Data Sovereignty Across the Automotive Value Chain with Catena-X

Digital Twins have evolved as a concept describing digital representations of physical assets. They can be used to facilitate simulations, monitoring, or optimization of product lifecycles. Considering the concept of a Circular Economy, which entails several lifecycles of, e.g., vehicles, their components, and materials, it is important to investigate how the respective Digital Twins are managed over the lifecycle of their physical assets. This publication presents and compares three approaches for managing Digital Twins in industrial use cases. The analysis considers aspects such as updates, data ownership, and data sovereignty. The results based on the research project Catena-X

==> literature.tex <==
\begin{thebibliography}{10}

    \bibitem{Stark2019}
    R.~Stark and T.~Damerau, ``Digital twin,'' in {\em {CIRP} Encyclopedia of
      Production Engineering} ({The International Academy for Production
      Engineering}, S.~Chatti, and T.~Tolio, eds.), (Berlin, Heidelberg), pp.~1--8,
      Springer Berlin Heidelberg, 2019.
    
    \bibitem{Grieves2018}
    M.~Grieves, ``The evolution of the digital twin,'' pp.~66--69, 2018.
    
    \bibitem{Grieves2022}
    M.~Grieves, ``Intelligent digital twins and the development and management of
      complex systems,'' vol.~2, p.~8, 2024.
    
    \bibitem{Grieves2016}
    M.~Grieves, ``Origins of the digital twin concept,'' vol.~8, 2016.
    
    \bibitem{CatenaX2024}
    Catena-X, ``Catena-x standard {CX} - 0002 {D}igital {}twins in {C}atena-{X}
      v.2.1.0,'' 2024.
    \newblock Accessed 22th March 2024.
    
    \bibitem{Muegge2022}
    J.~M{\"u}gge, I.~R. Hahn, T.~Riedelsheimer, and J.~Chatzis, ``Digital twins for
      circular economy - enabling decision support for r-strategies,'' {\em
      Industrie 4.0 Management}, vol.~2022, no.~6, pp.~42--46, 2022.
    
    \bibitem{Muegge2023}
    J.~Mügge, J.~G. Erdmann, T.~Riedelsheimer, M.~M. Manoury, S.-O. Smolka,
      S.~Wichmann, and K.~Lindow, ``Empowering end-of-life vehicle decision making
      with cross-company data exchange and data sovereignty via catena-x,''
      vol.~15, no.~9, p.~7187, 2023.
    
    \bibitem{Environment30.03.2022}
    {European Commission}, ``Proposal for ecodesign for sustainable products
      regulation,'' 2022.
    \newblock Accessed 05th May 2024.
    
    \bibitem{EPCEU12.07.2023}
    {European Parliament and Council of the European Union}, ``Regulation (eu)
      2023/1542 of the european parliament and of the council of 12 july 2023
      concerning batteries and waste batteries, amending directive 2008/98/ec and
      regulation (eu) 2019/1020 and repealing directive 2006/66/ec: Battery
      regulation,'' 2023.
    \newblock Accessed 10th May 2024.
    
    \bibitem{EuropeanCommission2020}
    {European Parliament and Council of the European Union}, ``Proposal for a
      regulation of the european parliament and of the council concerning batteries
      and waste batteries, repealing directive 2006/66/ec and amending regulation
      (eu) no 2019/1020,'' 2020.
    \newblock Accessed 05th May 2024.
    
    \bibitem{Potting2017}
    J.~Potting, M.~Hekkert, E.~Worrell, and A.~Hanemaaijer, ``Circular economy:
      Measuring innovation in the product chain,'' 2017.
    
    \bibitem{CatenaXAutomotiveNetworke.V..}
    {Catena-X Automotive Network e.V.}, ``Who is catena-x.''
    \newblock Accessed 11th May 2024.
    
    \bibitem{IndustrialDigitalTwinAssociation.June2023}
    {Industrial Digital Twin Association}, ``Asset administration shell
      specification: Part 2: Application programming interfaces,'' 2023.
    \newblock Accessed 01st May 2024.
    
    \bibitem{IndustrialDigitalTwinAssociation.March2023}
    {Industrial Digital Twin Association}, ``Asset administration shell
      specification: Part 1: Metamodel schema,'' 2023.
    \newblock Accessed 01st May 2024.
    
    \bibitem{TractusX2024}
    Tractus-X, ``{Tractus-X Industry Core KIT (Release 24.03)},'' 2024.
    
    \bibitem{Hellmeier2023}
    M.~Hellmeier and F.~von Scherenberg, ``A delimitation of data sovereignty from
      digital and technological sovereignty,'' no.~306, 2023.
    
    \bibitem{Jarke2019}
    M.~Jarke, B.~Otto, and S.~Ram, ``Data sovereignty and data space ecosystems,''
      vol.~61, no.~5, pp.~549--550, 2019.
    
    \bibitem{Scherenberg2024}
    F.~von Scherenberg, M.~Hellmeier, and B.~Otto, ``Data sovereignty in
      information systems,'' vol.~34, no.~1, 2024.
    
    \bibitem{Otto.2022}
    B.~Prof. Dr.-Ing.~Otto, S.~Steinbu{\ss}, A.~Teuscher, S.~Prof. Dr.~Auer,
      S.~Bader, H.~Bastiaansen, H.~Bauer, T.~Berthold, P.~Birnstil, M.~B{\"o}hmer,
      J.~Dr.~Bohn, G.~B{\"o}ge, R.~Brandst{\"a}tter, G.~Brost, J.~Ceballos,
      J.~Dr.-Ing.~Cirullies, C.~Ciureanu, E.~Corsi, S.~Dalmolen, S.~Danielsen,
      A.~Duisberg, A.~Eitel, T.~Ernst, K.~Fidomski, F.~Fournier, M.~Franz, M.~Gall,
      S.~Dr.~Geisler, J.~Gelhaar, R.~Gude, C.~Dr.-Ing~Haas, J.~Heiles, B.~Heisen,
      J.~Hierro, J.~Hoernle, A.~Hosseinzadeh, M.~Huber, M.~Huber, S.~Jiminez,
      C.~Jung, J.~Prof. Dr.~J{\"u}rjens, A.~Dr.~Kasprzik, M.~Dr.~Ketterl,
      J.~Koetzsch, J.~K{\"o}hler, C.~Dr.~Lange, D.~Langer, J.~Langkau, D.~Lis,
      S.~Dr.-Ing.~Lohmann, U.~Dr.~L{\"o}wen, C.~Dr.~Mader, B.~M{\"u}ller, N.~Mez,
      C.~Mertens, A.~M{\"u}ller, L.~Nagel, R.~Dr.~Nagel, H.~Nieminen,
      T.~Reitelbach, A.~Resetko, D.~Pakkala, J.~Pampus, F.~Patzer, H.~Pettenpohl,
      R.~Pietzsch, J.~Pullmann, M.~Punter, C.~Dr.~Quix, D.~Dr.~Rohrmus, L.~Romer,
      M.~{de Roode}, J.~Sandl{\"o}hken, P.~Sch{\"o}we, D.~Schulz,
      J.~Dr.~Sch{\"u}tte, K.~Dr.~Schweichhart, S.~Schwichtenberg, N.~Simon,
      I.~Skarbowski, E.-J. Prof.~Sol, P.~Sorowka, G.~Prof. Dr.-Ing.~Spiegelberg,
      M.~Spiekermann, C.~Spohn, G.~St{\"o}hr, E.~Tanger, M.~Dr.~The{\ss}, R.~Touma,
      S.~Dr.~Tramp, A.~Turkmayali, M.~Dr.~Wappler, A.-C. Weiergr{\"a}ber,
      S.~Dr.~Wenzel, A.~Wiencke, J.~Winkel, O.~W{\"o}lff, and H.~W{\"o}rner,
      ``Ids-ram 4.2,'' 2022.
    \newblock Accessed 01st May 2024.
    
    \bibitem{Manoury2023}
    M.~Manoury, ``Functional architecture for solution independent realization of
      digital continuity in system development,'' 2023.
    
    \bibitem{NationalArchives}
    {The National Archives}, ``What is digital continuity,'' 2017.
    \newblock Accessed 22th March 2024.
    
    \bibitem{Held.2021}
    M.~Held, N.~Rosat, G.~Georges, H.~Pengg, and K.~Boulouchos, ``Lifespans of
      passenger cars in europe: empirical modelling of fleet turnover dynamics,''
      {\em European transport research review}, vol.~13, no.~1, p.~9, 2021.
    
    \bibitem{VDI/VDE2021}
    {VDI/VDE 2206}, ``Development of mechatronic and cyber-physical systems,''
      2021.
    
    \bibitem{Riedelsheimer.b}
    T.~Riedelsheimer, L.~Dorfhuber, and R.~Stark, ``User centered development of a
      digital twin concept with focus on sustainability in the clothing industry,''
      {\em Procedia CIRP}, vol.~90, pp.~660--665, 2020.
    
    \bibitem{Riedelsheimer.2021}
    T.~Riedelsheimer, S.~Gogineni, and R.~Stark, ``Methodology to develop digital
      twins for energy efficient customizable iot-products,'' {\em Procedia CIRP},
      vol.~98, pp.~258--263, 2021.
    
    \bibitem{TractusX}
    Tractus-X, ``{Tractus-X EcoPass KIT (Release 24.03)},'' 2024.
    \newblock Accessed 25th March 2024.
    
    \bibitem{SAF14.03.2023}
    {Scaled Agile Framework}, ``About - scaled agile framework,'' 2023.
    
    \bibitem{KraftfahrtBundesamt.2024}
    Kraftfahrt-Bundesamt, ``Number of registered vehicles in germany,'' 2024.
    
    \bibitem{UmweltbundesamtUBA.2024}
    {Umweltbundesamt UBA}, ``End of life vehicles in germany (german:
      Altfahrzeugverwertung und fahrzeugverbleib),'' 2024.
    \newblock Accessed 10th May 2024.
    
    \bibitem{TractusX27.04.2024a}
    Tractus-X, ``{Tractus-X Digital Twin KIT (Release 24.03)},'' 2024.
    \newblock Accessed 27th April 2024.
    
    \bibitem{FOIS}
    {Federal Office for Information Security}, ``A brief guideline on
      self-sovereign identities with special regard to the distributed ledger
      technology,'' 2021.
    
    \bibitem{Hae.2022}
    H.~Ha{\ss}e, H.~{van der Valk}, F.~M{\"o}ller, and B.~Otto, ``Design principles
      for shared digital twins in distributed systems,'' {\em 1867-0202}, vol.~64,
      no.~6, pp.~751--772, 2022.
    
    \end{thebibliography}
    
